Visual Hallucination: Definition, Quantification, and Prescriptive Remediations

The troubling rise of hallucination presents perhaps the most significant impediment to the advancement of responsible AI. In recent times, considerable research has focused on detecting and mitigating hallucination in Large Language Models (LLMs). However, it's worth noting that hallucination is also quite prevalent in Vision-Language models (VLMs). In this paper, we offer a fine-grained discourse on profiling VLM hallucination based on two tasks: i) image captioning, and ii) Visual Question Answering (VQA). We delineate eight fine-grained orientations of visual hallucination: i) Contextual Guessing, ii) Identity Incongruity, iii) Geographical Erratum, iv) Visual Illusion, v) Gender Anomaly, vi) VLM as Classifier, vii) Wrong Reading, and viii) Numeric Discrepancy. We curate Visual HallucInation eLiciTation (VHILT), a publicly available dataset comprising 2,000 samples generated using eight VLMs across two tasks of captioning and VQA along with human annotations for the categories as mentioned earlier.

==> 3_VHVI.tex <==


%\vspace{-3mm}
\section{Visual Hallucination Vulnerability Index (VHVI)} \label{VHVI}
\vspace{-3mm}
With the increasing usage of VLMs and their tendency to hallucinate, there is a lack of uniform evaluation metrics to measure these hallucinations. To bridge this gap, we introduce VHVI, a comparative spectrum that enables us to assess and rank VLMs according to their susceptibility to generating hallucinations. We provide two VHVI metrics: one to assess hallucination related to image captioning and the second one to measure hallucination for VQA.

When defining VHVI, we take several factors into account. Firstly, not all captions/answers generated by a VLM are hallucinated, so it is important to determine the ratio of actual hallucinated captions/answers with the total number of captions/answers. In this context, we consider $U$ as the total number of captions/answers produced by a VLM. Moreover, VLMs can exhibit varying degrees of hallucination, including alarming, mild, and low types. For instance, if we have two VLMs and their total number of generated hallucinations in terms of captions/answers are the same, but VLM1 produces significantly more alarming hallucinations than VLM2, we must rank VLM1 higher in terms of VHVI. This comparative measure is achieved using multiplicative damping factors, $\delta_H$, $\delta_M$, and $\delta_L$ which are calculated based on $\mu \pm rank_x \times \sigma$. Initially, we calculate the HVI for all the VLMs, considering $\delta_H$, $\delta_M$, and $\delta_L$ as one. With these initial VHVIs, we obtain the mean ($\mu$) and standard deviation ($\sigma$), allowing us to recalculate the HVIs for all the LLMs. The resulting HVIs are then ranked and scaled providing a comparative spectrum as presented in equation \ref{eq:eq_1} and \ref{eq:eq_2}, similar to z-score normalization \cite{Normalization-z} and/or min-max normalization \cite{Normalization-min}. Having damping factors enables easy exponential smoothing with a handful of data points, 3/5 in this case. Finally, for ease of interpretability, VHVI is scaled between $0-100$. Figure \ref{fig:VHVI_Caption}, \ref{fig:VHVI_VQA} and \ref{fig:VHVI_categorywise_tasks} represents VHVI across tasks, models and categories.

\subsection{VHVI captioning}
When calculating $VHVI_{capt}$, we take into account the probability of each visual hallucination category. For example, $H_{CG}^C$ represents the total number of instances of Contextual Guessing out of the total $U$ generated captions. Therefore, the probability of this VLM generating Contextual Guessing-type hallucination is $(H_{CG}^C/U)$. %Equation \ref{eq:eq_1} represents the formula and figure \ref{fig:VHVI_Caption} and \ref{fig:VHVI_categorywise_tasks} represent models wise and category-wise visualization.
\vspace{-2mm}
\begin{equation} \label{eq:eq_1}
\resizebox{0.89\hsize}{!}{
\begin{split}
\Scale[0.8]{VHVI_{capt} = \frac{100}{U}[\sum_{x=1}^{U}(\delta_{H}*(H_{CG}^C+H_{II}^C+H_{GE}^C))+} \\
 \Scale[0.8]{(\delta_{M}*(H_{VI}^C+H_{GA}^C+H_{VC}^C))+(\delta_{L}*(H_{WR}^C+H_{ND}^C))]}
\end{split}}
\end{equation}


\vspace{-8mm}
\begin{figure}[!ht]
    \centering
\includegraphics[width=1\columnwidth]{Additional_Examples/VHVI_Captioning_Result-cropped.pdf}
\vspace{-7mm}
\caption{VHVI for VLM models based on captioning task using equation \ref{eq:eq_1}. The model size is found to be inversely proportional to VHVI.}
    \label{fig:VHVI_Caption}
\end{figure}


\vspace{-6mm}
\subsection{VHVI VQA}
When calculating $VHVI_{vqa}$, we take into account the probability of each visual hallucination category. For example, $H_{CG}^{vqa}$ represents the total number of instances of Contextual Guessing out of the total $U$ generated captions. Therefore, the probability of this VLM generating Contextual Guessing-type hallucination is $(H_{CG}^{vqa}/U)$.

\vspace{-4mm}

\begin{equation} \label{eq:eq_2}
\resizebox{0.89\hsize}{!}{
\begin{split}
 \Scale[0.8]{VHVI_{vqa} = \frac{100}{U*2}[\sum_{x=1}^{U}(\delta_{H}*H^{vqa}_{CG}+H^{vqa}_{II}+H^{vqa}_{GE}))+} \\
 \Scale[0.8]{(\delta_{M}*(H^{vqa}_{VI}+H^{vqa}_{GA}+H^{vqa}_{VC}))+(\delta_{L}*(H^{vqa}_{WR}+H^{vqa}_{ND}))]}
%\label{equation:equation2}
\end{split}
}
\end{equation}

\vspace{-6mm}
 
\begin{figure}[!ht]
    \centering
\includegraphics[width=1\columnwidth]{Additional_Examples/VHVI_VQA_Result-cropped.pdf}
\vspace{-4mm}
\caption{VHVI for VLM models based on VQA task using equation \ref{eq:eq_2}.}
    \label{fig:VHVI_VQA}
\end{figure}
\vspace{-2mm}

\begin{figure}[!ht]
    \centering
\includegraphics[width=0.95\columnwidth]{img/VHVI_graph_1.pdf}
\vspace{-3mm}
\caption{VHVI for different hallucination categories across various VLMs (see table \ref{tab:VHVI all}).}
    \vspace{-5mm}
\label{fig:VHVI_categorywise_tasks}
\end{figure}




\begin{tcolorbox}[
left=9pt,right=2pt,colback=teal!5!white,colframe=teal!75!black,colbacktitle=teal,
  title=\footnotesize \fontfamily{qbk} \selectfont \textbf{Implications derived from VHVI} ]
  
\vspace{-2mm}
\begin{itemize}
[labelindent=-0.2em,labelsep=0.1cm,leftmargin=*]
\setlength\itemsep{0em}
\begin{spacing}{0.85}

\item[\ding{224}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{8}{9}
%\begin{spacing}{1}
\selectfont

Alarming hallucination categories like contextual guessing, identity incongruity, geographic erratum, and visual illusion are prevalent in VLMs beyond a certain size. For instance, Kosmos-2 for image captioning, and InstructBLIP and LLaVa for VQA exhibit higher vulnerability to these alarming categories of hallucination.
}
%\end{spacing}
}

\item[\ding{224}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{8}{9}
%\begin{spacing}{1}
\selectfont

The numeric discrepancy, wrong reading, and VLM as a classifier are pervasive issues across all VLMs across both tasks.
}
}


\vspace{-6mm}
\end{spacing}
\end{itemize}
\end{tcolorbox}
\vspace{-2mm}
 


==> 4_MitigationTechnique.tex <==
\section{Mitigating Visual Hallucination - Baselines on \includegraphics[height=0.27cm,width=1.2cm]{img/VHILT.png}}
\vspace{-2mm}
While eliminating visual hallucination presents a complex challenge, this paper investigates three plausible directions for mitigation: (i) meta-learning (MeLa), (ii) visual contrastive decoding (VCD), and (iii) visual retrieval augmented generation. The reported results from these approaches can serve as baselines for future researchers. Figure \ref{fig:Impact_mitigation} describes the impact of the mitigation techniques. 

\vspace{-2mm}
\subsection{Meta Learning (MeLa)}
Inspired by \cite{tong2024eyes}, we have adopted the approach of leveraging CLIP and DINOv2 embeddings to improve image-text representation. This merging technique, commonly known as meta-learning, has been previously explored in both NLP \cite{Bollegala2018LearningWM, yin-schutze-2016-learning, Chen2013TheEP} and CV \cite{gao2022matters, 9428530} domains. In simplifying the integration of two different dimensional and non-aligned embeddings, an autoencoder-based approach appears to be the most plausible, as explored in previous research \cite{Bollegala2018LearningWM}. There are three families of autoencoding methods proposed in the literature: i) Decoupled Autoencoded Meta-Embedding (DAEME), ii) Concatenated Autoencoded Meta-Embedding (CAEME), and iii) Averaged Autoencoded Meta-Embedding (AAEME). We have experimented with all three and found AAEME to be the most suitable for this purpose. AAEME computes the meta-embedding of an \textit{object} from its two source embeddings $s1(o)$ and $s2(o)$ as the $l_2$-normalised (\textit{in our experiments we found $l_2$2-normalisation to improve performance}) sum of two encoded versions of the source embeddings $E_1(s_1(o))$ and $E_2(s_2(o))$, given by $m(o)=\frac{E_{1}(S_1(o))+E_{2}(S_2(o))}{\left \| E_{1}(S_1(o))+E_{2}(S_2(o) \right \|_{2}}$.
%If we do that, what are the categories getting affected? which categories benefit more The CLIP\cite{radford2021learning} + DINO \cite{caron2021emerging} method merges the capabilities of CLIP and DINOv2 embeddings to enhance image interpretation in multimodal language models. It operates by concurrently processing images through both CLIP and DINOv2 encoders and refining their features independently. The refined information from both sources is then integrated in a coherent manner to improve the model's understanding of visual content. This approach facilitates better alignment between visual and linguistic information, thereby enhancing the model's performance in tasks involving image understanding and description. 

%Affect of CLIP+DINO on caption categories 

%Affect of CLIP + DINO on VQA



\subsection{Visual Contrastive Decoding (VCD)}

%kosmos-2 2 -3 evaluation metrics to study grounding [krishnav - 5 evaluation metrics for grounding]
%Kosmos Metric -The model predicts the locations of phrases within captions, generating location tokens in "<box>...</box>" format, which are then converted into bounding boxes. Correct bounding boxes are determined by an intersection over union (IoU) threshold of 0.5 with ground-truth bounding boxes. Evaluation metrics include recall at top 1, 5, and 10 bounding boxes (R@1, R@5, R@10), calculated based on the generated bounding boxes.

%Another evaluation method would be on REC benchmarks including RefCOCO, RefCOCO+ and RefCOCOg datasets. REC benchmarks evaluate models' ability to comprehend referring expression, requiring accurate localization of objects referenced in textual descriptions within images. The evaluation metrics for REC benchmarks typically include measures such as accuracy and precision in localizing the referred objects.

We drew inspiration from \cite{leng2023mitigating} and utilized their implementation. Additionally, we incorporated the CalTech Similar Object dataset for VCD training. The aim here is to train VLMs to better distinguish similar-looking objects. Our setup is as follows. Suppose that we have a pair ($I_i,I_j$) e.g., image samples of the term \textit{building} and a label Y (the term \textit{building} in the text) that is equal to $0$ if the samples are similar and $1$ otherwise. To extract a low-dimensional representation of each sample, we finetune VLM with $f$ that encodes the input images $I_i$ and $I_j$ into an embedding space where $x_i=f(I_i)$ and $x_j=f(I_j)$. The contrastive loss is defined as $L = (1-Y) * | x_i-x_j|2+Y * max(0, m-| x_i-x_j|^2 )$, where $m$ is a hyperparameter, defining the lower bound distance between dissimilar samples.
\vspace{-1.5mm}
\subsection{Visual RAG} \label{subsection : Visual RAG}  %anku
Drawing inspiration from the significant popularity of RAG in correcting or mitigating factual information for LLMs, we have incorporated RAG specifically for two categories: 1) Identity Incongruity and 2) Geographic Erratum. In these cases, when the VLM generates any Named Entity (NE), such as a person's name or a location name, we automatically identify them and search them in Google. The retrieved top image results are then matched with the original image, and if the overall match exceeds an experimentally determined threshold, we consider it correct; otherwise, it is considered incorrect. We observed that approximately $30\%$ of cases resulted in all VLMs being incorrect for these two categories. For measuring image similarity, we utilized this library \cite{yokoo2021contrastive}, winner of the Facebook AI Image Similarity Challenge 2019.

\vspace{-3mm}
%%%%%%%%%%%%%%%%%%%%%
\begin{tcolorbox}[
left=9pt,right=2pt,colback=brown!5!white,colframe=brown!75!black,colbacktitle=brown,
  title=\footnotesize \fontfamily{qbk} \selectfont \textbf{Takeaway from Mitigation baselines} ]
  
\vspace{-2mm}
\begin{itemize}
[labelindent=-0.2em,labelsep=0.1cm,leftmargin=*]
\setlength\itemsep{0em}
\begin{spacing}{0.85}

\item[\ding{224}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{8}{9}
%\begin{spacing}{1}
\selectfont

MeLa has exhibited significant improvements solely in the realm of caption hallucination for the VLM Kosmos-2 across three classes: Visual Illusion, Geographic Erratum, and Contextual Guessing. However, MeLa's performance enhancements in certain cases for VQA were only marginal.
}
%\end{spacing}
}

\item[\ding{224}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{8}{9}
%\begin{spacing}{1}
\selectfont
VCD has demonstrated notable performance improvements in two hallucination categories, namely "VLM as classifier" and "Gender Anomaly," specifically in the caption hallucination task for only one VLM, Spinx-1K. Regarding VQA hallucination, VCD has exhibited superior performance in the same two tasks for MultimodalGPT.
}
}

\item[\ding{224}] 
{\footnotesize 
{\fontfamily{phv}\fontsize{8}{9}
%\begin{spacing}{1}
\selectfont
Visual RAG has exhibited impressive performance in the caption hallucination task for Kosmos-2, particularly excelling in two categories: "Geographic Erratum" and "Identity Incongruity." Moreover, it appears to be effective in addressing the same two categories for VQA hallucination in models such as MiniGPT-4, LLaVa, and InstructBLIP.}
}


\vspace{-6mm}
\end{spacing}
\end{itemize}
\end{tcolorbox}
\vspace{-2mm}
 





%%%%%%%%%%%%%%%%%%%%%%






%caption - google search - 10 results - bad number

%although similarity based isn't good, it is apparent that this kind of 

%image similarity SOTA

%In the field of NLP, textual entailment recognition involves determining, from two text fragments, whether the meaning of one text can be logically inferred from another. Although it can be challenging to detect hallucinations in LLMs, TE is an effective technique to detect the factuality of a given text by looking up web sources. However, there are certain limitations of the current TE approaches. One straightforward approach to detect hallucination in an LLM-generated response is by looking it up on the updated sources of the web using TE. The three possible outcomes of any TE method are: \textit{i) support},  \textit{ii) refute}, and, \textit{iii) not enough information}. Using these scores, whether hallucination exists or not could be determined. For scores containing support, there is \textit{no} hallucination, whereas refute scores indicate hallucination. Despite using these scores for detection, they still are not sufficient because all support scores necessarily do not mean an absence of hallucination and vice-versa. 

==> 5_HallucinationMitigation.tex <==
\input{table/fig_8}

\section{Mitigation methods}

Visual hallucination poses a significant challenge in large multi-modal models (LMMs) and large vision-language models (LVLMs), where generated outputs may deviate from accurate representations of the input data. To address this issue, researchers have developed innovative mitigation methods aimed at enhancing the robustness and reliability of these models.  This section provides an overview of all the approaches designed to alleviate visual hallucination through distinct strategies. 
\begin{enumerate}
    \item The paper \textit{"Mitigating Object Hallucinations in Large Vision-Language Models through Visual Contrastive Decoding"} \cite{leng2023mitigating} proposes a novel method called Visual Contrastive Decoding (VCD). VCD tackles object hallucinations by introducing controlled uncertainty into the input image through Gaussian noise. This technique encourages the model to focus on the most salient visual features and reduce reliance on statistical biases or unimodal priors, which are often responsible for hallucinations. VCD operates in three key stages:
    \begin{enumerate}
        \item \textbf{Noise injection:} Gaussian noise is added to the original input image, creating a distorted version. 
        \item \textbf{Dual-stream decoding:} The LVLM generates two sets of textual outputs, one for the original and one for the distorted image. 
        \item \textbf{Contrastive distribution and sampling:} A contrastive distribution is calculated by comparing the probabilities of each word across both outputs. This distribution is then used to sample the final model output, favoring words that are consistent with both the original and distorted images. 
    \end{enumerate}
    
The authors conducted extensive experiments on various LVLM families and demonstrated the effectiveness of VCD in mitigating object hallucinations. Notably, VCD achieved significant reductions in hallucination rates across all models without requiring any additional training or external tools. Moreover, VCD led to consistent improvements in perception-based tasks, such as object detection and image captioning, while maintaining the original recognition capabilities of the LVLMs. These findings suggest that VCD has the potential to go beyond hallucination mitigation and enhance the overall robustness and reliability of LVLMs. 
    \item \textit{"Detecting and Preventing Hallucinations in Large Vision Language Models"} \cite{gunjal2023detecting} introduces M-HalDetect, a comprehensive multi-modal hallucination detection dataset for detailed image descriptions. The authors also propose a novel Fine-grained Direct Preference Optimization (FDPO) and fine-grained multi-modal reward models to prevent hallucinations in LVLMs. 
M-HalDetect stands out for its granular annotations on 16,000 VQA examples, surpassing previous datasets by providing nuanced insights into hallucination occurrences within generated descriptions. Unlike its predecessors, M-HalDetect allows for sub-sentence analysis, pinpointing the precise locations of hallucinations. This granularity facilitates a more focused analysis, enabling the development of targeted mitigation strategies for Language and Vision Models (LVMs). 

The paper further introduces two novel mitigation strategies: Fine-grained Multimodal Reward Models and Fine-grained Direct Preference Optimization (FDPO), leveraging M-HalDetect's detailed annotations. Reward models act as coaches, guiding LVLMs during training to emphasize accuracy and discourage hallucinations. FDPO, a direct training approach, focuses on individual LVLM outputs, aligning them with M-HalDetect's annotations to teach models to avoid hallucinations. Both strategies, rooted in M-HalDetect's rich annotations, collaboratively aim to reduce hallucinations and enhance LVLMs' ability to generate truthful and reliable image descriptions, significantly advancing their robustness in real-world applications. 
\item \textit{Plausible May Not Be Faithful: Probing Object Hallucination in Vision-Language Pre-training} \cite{dai2022plausible} systematically study the problem of Object Hallucination in vision-language pre-training (VLP) models, by examining recent state-of-the-art VLP models, investigating different types of image encoding, and proposing a new VLP loss called Object Masked Language Modeling (ObjMLM) to mitigate object hallucination. They show that even the best-performing VLP models still hallucinate frequently and that the widely used optimization method Self-Critical Sequence Training (SCST) can lead to more hallucination. 

The authors propose ObjMLM as a simple yet effective pre-training objective to improve object-level image-text alignment and reduce object hallucination. ObjMLM aims to improve object-level image-text alignment by enhancing the controllability of vision-conditioned text generation. It can be seen as a variant of the Masked Language Modeling (MLM) loss, where all the objects in the text that appear in the image are masked. By doing so, ObjMLM indirectly controls the model to only generate objects that are visible in the input image, thus reducing the generation of non-existent or incorrect objects. Additionally, ObjMLM enhances the model's recognition ability when describing the spatial relationship between objects, which is a common scenario that causes hallucinations frequently. Experimental results show that ObjMLM reduces object hallucination by 17.4\% without introducing extra training data, demonstrating its effectiveness in mitigating the problem of object hallucination in VLP models.
\item \textit{Woodpecker: Hallucination Correction for Multimodal Large Language Models} \cite{yin2023woodpecker} introduces a training-free method, Woodpecker, designed to correct hallucinations in responses generated by Multimodal Large Language Models (MLLMs) without requiring retraining. The key objective of Woodpecker is to refine the responses of MLLMs by modifying the hallucinated parts, thereby improving the factuality of the generated content. Unlike existing studies that mainly resort to instruction-tuning and retraining models with specific data to mitigate hallucinations, Woodpecker takes a different approach by incorporating a five-stage framework: key concept extraction, question formulation, visual knowledge validation, visual claim generation, and hallucination correction. This method aims to diagnose and correct hallucinations in the response generated by MLLMs, providing a training-free and interpretable solution. The method consists of five stages:
\begin{enumerate}
                    \item \textbf{Key concept extraction:} Identifying the main objects mentioned in the generated sentences. 
                    \item \textbf{Question formulation:} Asking questions around the extracted objects, such as their number and attributes. 
                    \item \textbf{Visual knowledge validation:} Answering the formulated questions via expert models, such as visual perception models.
                    \item \textbf{Visual claim generation: }Converting the Question-Answer (QA) pairs into a visual knowledge base, consisting of object-level and attribute-level claims about the input image. 
                    \item \textbf{Hallucination correction: }Modifying the hallucinations in the enerated text and adding corresponding evidence, such as bounding boxes. 
\end{enumerate}
Woodpecker's approach exempts the complexity of collecting instruction data and resource-intensive training, making it easily integrable with various MLLMs, serving as a general plug-and-play module . The method focuses on leveraging the strong reasoning and language proficiencies of LLMs to help with key concept extraction, question formulation, and hallucination correction . By incorporating visual knowledge validation and claim generation, Woodpecker provides interpretability and reliability beyond the black-box MLLMs, offering convenient visual fact-checking. The paper evaluates Woodpecker both quantitatively and qualitatively, demonstrating its potential in correcting hallucinations and improving accuracy over baseline models.
\item \textit{Mitigating Hallucination in Large Multi-Modal Models via Robust Instruction Tuning} \cite{liu2023aligning}  addresses the issue of hallucination in large multi-modal models (LMMs) by introducing the Large-scale Robust Visual (LRV)-Instruction dataset, which comprises 400k visual instructions covering 16 vision-and-language tasks. The dataset includes both positive and negative instructions for more robust visual instruction tuning. To evaluate visual instruction tuning, the authors propose GPT4-Assisted Visual Instruction Evaluation (GAVIE), a stable approach that does not require human-annotated ground truth answers and can adapt to diverse instruction formats. 

The GAVIE method works by leveraging GPT4 to evaluate the output from current LMMs in the context of visual instruction tuning. GAVIE assesses the relevancy and accuracy of the LMMs' responses to human instructions without requiring human-annotated ground-truth answers and pre-designed instruction formats. It does so by providing GPT4 with the image content and human instructions and then asking GPT4 to score the responses from the LMMs based on their relevance and accuracy.

The authors also demonstrate that existing LMMs exhibit significant hallucinations when presented with negative instructions, particularly Existent Object and Knowledge Manipulation instructions. To mitigate hallucination, the authors fine-tune MiniGPT4 and mPLUG-Owl on LRV-Instruction, leading to improved performance on several public datasets compared to state-of-the-art methods. The LRV-instruction dataset includes both positive and negative instructions, designed at three semantic levels: Nonexistent Object Manipulation, Existent Object Manipulation, and Knowledge Manipulation. By incorporating both positive and negative instructions in the finetuning process, the authors aimed to train the LMMs to respond more faithfully to human instructions and reduce the occurrence of hallucination. This approach allowed the models to learn to differentiate between various types of instructions and generate more accurate and relevant responses, ultimately improving their robustness in following human instructions and reducing hallucination. They observed that a balanced ratio of positive and negative instances in the training data leads to a more robust model. 
\item \textit{Analyzing and Mitigating Object Hallucination in Large Vision-Language Models} \cite{zhou2023analyzing}
presents a comprehensive analysis of object hallucination in large vision-language models (LVLMs) and introduces the LVLM Hallucination Revisor (LURE) algorithm to address this issue. LURE is designed to rectify object hallucination by revising the generated descriptions to align more closely with the actual content of the images. The algorithm leverages a combination of visual and linguistic cues to identify and correct hallucinated objects in the model's outputs. LURE is grounded in a rigorous statistical analysis of the key factors underlying object hallucination, including co-occurrence patterns (objects that frequently appear together), uncertainty in the model's predictions, and the position of objects within the image.  

To create the revisor, the authors first generate a hallucinatory dataset using GPT-3.5 by making two modifications to the original correct captions. First, they insert additional object texts into the description that are likely to co-occur with the objects contained in the initial description. This modification allows LURE to learn to disentangle such co-occurrence patterns effectively. Second, they replace uncertain objects or those at the end of descriptions with a placeholder tag, encouraging the revisor to re-evaluate these objects. 

Once trained on the hallucinatory dataset, the revisor can seamlessly integrate with any LVLM to correct potential hallucinatory descriptions. The algorithm leverages a combination of visual and linguistic cues to identify and correct hallucinated objects in the model's outputs. The evaluation of LURE on six open-source LVLMs demonstrated significant improvements in mitigating general object hallucination. The results showed a 23\% improvement in general object hallucination evaluation metrics over the previous best approach. Additionally, in both GPT evaluation and human evaluation, LURE consistently ranked at the top, indicating its effectiveness in reducing object hallucination in the generated descriptions produced by LVLMs. 
\item \textit{Volcano: Mitigating Multimodal Hallucination through Self-Feedback Guided Revision} \cite{lee2023volcano} leverages self-feedback to mitigate multimodal hallucination in large multimodal models. The proposed method, VOLCANO, leverages natural language feedback and visual information to enable the model to correct hallucinated responses. 

VOLCANO is a multimodal self-feedback guided revision model designed to effectively mitigate multimodal hallucination. The method is trained to generate an initial response based on the given image and question, and then sequentially revises it until no further improvement is deemed necessary. This iterative refinement process is guided by self-feedback, which allows the model to correct hallucinated responses by offering detailed visual information. 

VOLCANO addresses multimodal hallucination by utilizing natural language feedback to guide the model in revising its responses. The feedback generated by VOLCANO is rooted in the image and conveys rich visual details, providing essential guidance to reduce multimodal hallucination, even in cases where the vision encoder inadequately grounds the image. This approach effectively tackles the challenge of multimodal hallucination by leveraging the power of self-feedback to refine and improve model responses based on visual cues.
\end{enumerate}



==> table/MeLa_VHVI_VQA.tex <==
\begin{table}
\label{tab-VHVI_MeLa_VQA}
\centering
\footnotesize
\begin{tabular}{lccccccccc}
\toprule
Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
mPlugOwl & 53 & 59 & 52 & 49 & 65 & 22 & 14 & 11 \\
MultiModel-GPT & 50 & 52 & 55 & 40 & 62 & 24 & 12 & 13 \\
MiniGPT-4 & 48 & 56 & 30 & 25 & 67 & 26 & 17 & 12 \\
LLaVa & 54 & 48 & 30 & 30 & 52 & 32 & 15 & 12 \\
InstructBLIP & 47 & 40 & 26 & 22 & 44 & 30 & 19 & 15 \\
\bottomrule
\end{tabular}
\caption{Effect of Meta Learning (MeLa) on VHVI score for VQA models}
\end{table}


==> table/MeLa_VHVI_caption.tex <==
\begin{table}
\label{tab-VHVI_MeLa_caption}
\centering
\footnotesize
\begin{tabular}{lccccccccc}
\toprule
Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
Sphinx-1k & 56 & 58 & 46 & 48 & 69 & 23 & 12 & 28 \\
MiniGPT-v2 & 48 & 52 & 33 & 34 & 66 & 28 & 18 & 32 \\
Kosmos-2 & 31 & 45 & 18 & 18 & 49 & 36 & 32 & 31 \\
\bottomrule
\end{tabular}
\caption{Effect of Meta Learning (MeLa) on VHVI score for Captioning models}
\end{table}

==> table/VCD_VHVI_caption.tex <==
\begin{table}
\label{tab-VHVI_VCD_caption}
\centering
\footnotesize
\begin{tabular}{lccccccccc}
\toprule
Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
Sphinx-1k & 56 & 58 & 35 & 36 & 69 & 23 & 12 & 28 \\
MiniGPT-v2 & 48 & 52 & 26 & 28 & 66 & 28 & 18 & 32 \\
Kosmos-2 & 31 & 45 & 17 & 18 & 58 & 46 & 34 & 39 \\
\bottomrule
\end{tabular}
\caption{Effect of Visual Contrastive Decoding (VCD) on VHVI score for Captioning models}
\end{table}

==> table/VHVI_score_VQA.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{lccccccccc}
\toprule
Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
mPlugOwl & 53 & 59 & 56 & 52 & 70 & 22 & 14 & 36 \\
MultiModel-GPT & 50 & 52 & 59 & 43 & 66 & 24 & 12 & 32 \\
MiniGPT-4 & 48 & 56 & 36 & 29 & 69 & 26 & 17 & 29 \\
LLaVa & 54 & 48 & 32 & 31 & 57 & 34 & 16 & 22 \\
InstructBLIP & 47 & 40 & 30 & 26 & 48 & 33 & 19 & 20 \\
\bottomrule
\end{tabular}
\caption{VHVI Score of different models on VQA task}
\label{tab-vhvi_vqa}
\end{table}

==> table/VHVI_score_VQA_Caption.tex <==
\begin{table*}[!htp]
\centering
\addtolength{\tabcolsep}{-3pt} 
\small
\begin{tabular}{lccccccccc}
\toprule
Task & Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& &Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
\multirow{3}{*}{Captioning} & Sphinx-1k & 56 & 58 & 46 & 48 & 69 & 23 & 12 & 28 \\
& MiniGPT-v2 & 48 & 52 & 33 & 34 & 66 & 28 & 18 & 32 \\
& Kosmos-2 & 31 & 45 & 21 & 24 & 58 & 46 & 34 & 39 \\
\midrule
\multirow{4}{*}{VQA} & mPlugOwl & 53 & 59 & 56 & 52 & 70 & 22 & 14 & 36 \\
& MultiModel-GPT & 50 & 52 & 59 & 43 & 66 & 24 & 12 & 32 \\
& MiniGPT-4 & 48 & 56 & 36 & 29 & 69 & 26 & 17 & 29 \\
& LlaVa & 54 & 48 & 32 & 31 & 57 & 34 & 16 & 22 \\
& InstructBLIP & 47 & 40 & 30 & 26 & 48 & 33 & 19 & 20 \\
\bottomrule
\end{tabular}
\caption{VHVI score of different models on captioning and VQA task}
\label{tab:VHVI all}
\end{table*}

==> table/VHVI_score_captionaing.tex <==
% VHVI
\begin{table}
\centering
\footnotesize
\begin{tabular}{lccccccccc}
\toprule
Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
& Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
Sphinx-1k & 56 & 58 & 46 & 48 & 69 & 23 & 12 & 28 \\
MiniGPT-v2 & 48 & 52 & 33 & 34 & 66 & 28 & 18 & 32 \\
Kosmos-2 & 31 & 45 & 21 & 24 & 58 & 46 & 34 & 39 \\
\bottomrule
\end{tabular}
\caption{VHVI Score of different models on captioning task}
\label{tab-vhvi_caption}
\end{table}

==> table/fig_8.tex <==
\begin{figure*}[!ht]
    \centering
\includegraphics[width=1\textwidth]{img/hallucination_mitigation.pdf}
\caption{Impact of mitigation techniques across the various categories and types of task.}
    \label{fig:VHVI_Caption}
\end{figure*}

==> table/mitigation_caption.tex <==
\begin{table*}[!htp]
\centering
\addtolength{\tabcolsep}{-3pt} 
\small
\begin{tabular}{lccccccccc}
\toprule
Mitigation & Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
Technique & &Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
\multirow{3}{*}{MeLa} & Sphinx-1k & 56 & 58 & 46 & 48 & 69 & 23 & 12 & 28 \\
& MiniGPT-v2 & 48 & 52 & 33 & 34 & 66 & 28 & 18 & 32 \\
& Kosmos-2 & 31 & 45 & 18 & 18 & 49 & 36 & 32 & 31 \\
\midrule
\multirow{3}{*}{VCD} & Sphinx-1k & 56 & 58 & 35 & 36 & 69 & 23 & 12 & 28 \\
& MiniGPT-v2 & 48 & 52 & 26 & 28 & 66 & 28 & 18 & 32 \\
& Kosmos-2 & 31 & 45 & 17 & 18 & 58 & 46 & 34 & 39 \\
\midrule
\multirow{3}{*}{Visual RAG} & Sphinx-1k & 56 & 58 & 46 & 48 & 69 & 18 & 8 & 28 \\
& MiniGPT-v2 & 48 & 52 & 33 & 34 & 66 & 19 & 10 & 32 \\
& Kosmos-2 & 31 & 45 & 21 & 24 & 58 & 22 & 12 & 39 \\
\bottomrule
\end{tabular}
\caption{Effect of different mitigation techniques on VHVI score for Captioning task}
\label{tab:VHVI caption mitigation}
\end{table*}


==> table/mitigation_vqa.tex <==
\begin{table*}[!htp]
\centering
\addtolength{\tabcolsep}{-3pt} 
\small
\begin{tabular}{lccccccccc}
\toprule
Mitigation & Model & Numeric &  Wrong & VLM as & Gender & Visual & Geographic  & Identity & Contextual \\
technique & &Discrepancy & Reading & Classifier & Anomaly & Illusion & Erratum & Incongruity & Guessing\\
\midrule
\multirow{4}{*}{MeLa} & mPlugOwl & 53 & 59 & 52 & 49 & 65 & 22 & 14 & 11 \\
& MultiModel-GPT & 50 & 52 & 55 & 40 & 62 & 24 & 12 & 13 \\
& MiniGPT-4 & 48 & 56 & 30 & 25 & 67 & 26 & 17 & 12 \\
& LlaVa & 54 & 48 & 30 & 30 & 52 & 32 & 15 & 12 \\
& InstructBLIP & 47 & 40 & 26 & 22 & 44 & 30 & 19 & 15 \\
\midrule
\multirow{4}{*}{VCD} & mPlugOwl & 53 & 59 & 48 & 46 & 70 & 22 & 14 & 11 \\
& MultiModel-GPT & 50 & 52 & 48 & 28 & 66 & 24 & 12 & 13 \\
& MiniGPT-4 & 48 & 56 & 27 & 21 & 69 & 26 & 17 & 18 \\
& LlaVa & 54 & 48 & 26 & 29 & 57 & 34 & 16 & 12 \\
& InstructBLIP & 47 & 40 & 21 & 22 & 48 & 33 & 19 & 20 \\
\midrule
\multirow{4}{*}{Visual RAG} & mPlugOwl & 53 & 59 & 56 & 52 & 70 & 18 & 8 & 36 \\
& MultiModel-GPT & 50 & 52 & 59 & 43 & 66 & 18 & 7 & 32 \\
& MiniGPT-4 & 48 & 56 & 36 & 29 & 69 & 19 & 5 & 29 \\
& LlaVa & 54 & 48 & 32 & 31 & 57 & 24 & 5 & 22 \\
& InstructBLIP & 47 & 40 & 30 & 26 & 48 & 20 & 6 & 20 \\
\bottomrule
\end{tabular}
\caption{Effect of different mitigation techniques on VHVI score for VQA task}
\label{tab:VHVI VQA mitigation}
\end{table*}

==> table/numbers_dataanalysis.tex <==
\begin{table*}[!htp]
\centering
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{lcc}
\hline
Category                                                    & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}No. of datapoints\\ for Captioning\end{tabular}} & \begin{tabular}[c]{@{}c@{}}No. of datapoints\\ for VQA\end{tabular} \\ \hline
No Hallucination                                            & 19639                                                                                             & 31904                                                                   \\
Contextual Guessing                                         &  10934                                                                                           &   17990                                                                \\
Indentity Incongruity                                       & 3496                                                                                              & 19084                                                                   \\
Geographical Erratum                                        & 27854                                                                                              & 17598                                                                   \\
Visual Illusion                                             & 8763                                                                                              & 13959                                                                  \\
Gender Anomaly                                              & 5478                                                                                             &  24843                                                                  \\
%\begin{tabular}[c]{@{}l@{}}VLM as\\ Classifier\end{tabular} & 7654                                                                                             & 13859                                                                  \\
VLM as Classifier                                               & 7654                                                                                            & 13859                                                                  \\
Wrong Reading                                               & 3393                                                                                            & 20324                                                                  \\
Numeric Discrepancy                                         & 17789                                                                                             & 15439                                                                 \\ \hline
Total                                                       & 105000                                                                                            & 175000                                                                  \\ \hline
\end{tabular}}
\caption{The table represents a breakdown of total datapoints for each category. }
\label{tab:Data Analysis}
\end{table*}
